VisualCheXbert: Addressing the Discrepancy Between Radiology Report Labels and Image Labels

Automatic extraction of medical conditions from free-text radiology reports is critical for supervising computer vision models to interpret medical images. In this work, we show that radiologists labeling reports significantly disagree with radiologists labeling corresponding chest X-ray images, which reduces the quality of report labels as proxies for image labels. We develop and evaluate methods to produce labels from radiology reports that have better agreement with radiologists labeling images. Our best performing method, called VisualCheXbert, uses a biomedically-pretrained BERT model to directly map from a radiology report to the image labels, with a supervisory signal determined by a computer vision model trained to detect medical conditions from chest X-ray images. We find that VisualCheXbert outperforms an approach using an existing radiology report labeler by an average F1 score of 0.14 (95% CI 0.12, 0.17). We also find that VisualCheXbert better agrees with radiologists labeling chest X-ray images than do radiologists labeling the corresponding radiology reports by an average F1 score across several medical conditions of between 0.12 (95% CI 0.09, 0.15) and 0.21 (95% CI 0.18, 0.24).

==> tables/old_rad_examples.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
\centering
\caption{\label{tab:report_examples} Clinical explanations of disagreements between radiologists looking at reports and radiologists looking at images on the CheXpert test set. Given access to the X-ray image, the full radiology report, the radiology report impression, the radiology report labels, and the image ground truth, a board-certified radiologist explained disagreements between radiologist report labels and the image ground truth. We show select examples with explanations in this table.}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Report Impression}                                                                                                                                                                                                                                                                                                                                                                                                                           & \textbf{Radiologist Report Label}                  & \textbf{Image Ground Truth}                        & \textbf{Clinical Explanation}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ \hline
\begin{tabular}[c]{@{}l@{}}1. single ap upright view of the chest showing a mildly increased\\ opacity at the left lung base that could represent atelectasis\\ versus consolidation.\end{tabular}                                                                                                                                                                                                                              & Negative for Cardiomegaly     & Positive for Cardiomegaly     & \begin{tabular}[c]{@{}l@{}}The radiologist looking at the report marks cardiomegaly \\ as negative as it is not mentioend in the report.  Since the \\ image is a Intensive Care Unit (ICU) film and cardiomegaly \\ is not a clinically relevant condition for the population selected \\ for in ICU films, the presence of cardiomegaly was never \\ mentioned in the report, resulting in the discrepancy between \\ radiologists looking at the report and radiologists looking \\ at the image.\end{tabular} \\ \hline
\begin{tabular}[c]{@{}l@{}}1. pulmonary vascular congestion. left lower lobe opacity\\ compatible with atelectasis and/or consolidation.\end{tabular}                                                                                                                                                                                                                                                                           & Negative for Cardiomegaly     & Positive for Cardiomegaly     & \begin{tabular}[c]{@{}l@{}}Although cardiomegaly was mentioned in the radiology report \\ findings section, cardiomegaly was not mentioned in the report \\ impression. Since the radiologist looking at the report only had \\ access to the impression section, they labeled cardiomegaly as negative \\ when it was actually present in the image.\end{tabular}                                                                                                                                              \\ \hline
\begin{tabular}[c]{@{}l@{}}1.  decreased pulmonary edema.  stable bilateral pleural effusions \\ and bibasilar atelectasis.\end{tabular}                                                                                                                                                                                                                                                                                        & Positive for Edema            & Negative for Edema            & \begin{tabular}[c]{@{}l@{}}The phrase "decreased pulmonary edema" shows that the radiologist \\ writing the report had relevant clinical context, as the edema has \\ "decreased" compared to a previous report or image. However, the \\ radiologist looking at the image does not have this clinical context, \\ resulting in a discrepancy.\end{tabular}                                                                                                                                                        \\ \hline
\begin{tabular}[c]{@{}l@{}}1.  single frontal radiograph of the chest is limited secondary to \\ poor inspiration and rotation.  \\ 2.  cardiac silhouette is partially obscured secondary to rotation.  \\ lungs demonstrate bibasilar opacities, likely reflecting atelectasis. \\ possible small right pleural effusion.  no pneumothorax.  \\ 3.  visualized osseous structures and soft tissues unremarkable.\end{tabular} & Positive for Pleural Effusion & Negative for Pleural Effusion & \begin{tabular}[c]{@{}l@{}}The phrase "possible small right pleural effusion" indicates the \\ uncertainty regarding the presence of pleural effusion. This natural \\ uncertainty may explain the disagreement between radiologists \\ looking at the image and radiologists looking at the report. Our \\ board-certified radiologist also noted that pleural effusion was \\ borderline in this example.\end{tabular}                                                                                          \\ \hline \begin{tabular}[c]{@{}l@{}}1. crowding of the pulmonary xclude mild\\ interstitial pulmonary edema.\\ 2. no focal air space consolidation. the cardiomediastinal\\ silhouette appears grossly within normal limits.\end{tabular}                                                                                                                                                                           & Negative for Pleural Effusion & Positive for Pleural Effusion & \begin{tabular}[c]{@{}l@{}}Our radiologist spotted an error in the radiology report, which did \\ not mention the presence of pleural effusion. This error in the report \\ itself may explain the disagreement between the image and report labels.\end{tabular}                                                                                                                                                                                                                                                 \\ \hline
\end{tabular}%
}
\end{table*}

==> tables/vingroup.tex <==
\begin{table}[t!]
\centering
\caption{\label{tab:vingroup} F1 scores obtained by BERT+LogReg trained on the MIMIC-CXR dataset, with labels provided by a DenseNet-121 or the higher-performing ResNeXt-50 model with MoCo v2 pretraining.}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcc}
\textbf{\begin{tabular}[c]{@{}l@{}}Condition \\ (n = \# positive)\end{tabular}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}BERT+LogReg on \\ MIMIC-CXR,\\ DenseNet labels\end{tabular}}} & \multicolumn{1}{l}{\textbf{\begin{tabular}[c]{@{}l@{}}BERT+LogReg on\\ MIMIC-CXR,\\ ResNeXt-50 labels \\ (VisualCheXbert)\end{tabular}}} \\ \hline
Atelectasis (n=153) & 0.64 & \textbf{0.67} \\
Cardiomegaly (n=151) & \textbf{0.62} & \textbf{0.62} \\
Edema (n=78) & \textbf{0.54} & 0.53 \\
Pleural Effusion (n=104) & 0.65 & \textbf{0.68} \\
Enlarged Cardiom. (n=253) & \textbf{0.73} & 0.72 \\
Lung Opacity (n=264) & 0.83 & \textbf{0.84} \\
Support Devices (n=261) & 0.87 & \textbf{0.88} \\
No Finding (n=62) & 0.54 & \textbf{0.55} \\ \hline
Average & 0.68 & \textbf{0.69} \\
Weighted Average & 0.73 & \textbf{0.74}
\end{tabular}%
}
\end{table}
